Limitations on counting in Boolean circuits and self-assembly

In self-assembly, a $k$-counter is a tile set that grows a horizontal ruler from left to right, containing $k$ columns each of which encodes a distinct binary string. Counters have been fundamental objects of study in a wide range of theoretical models of tile assembly, molecular robotics and thermodynamics-based self-assembly due to their construction capabilities using few tile types, time-efficiency of growth and combinatorial structure. Here, we define a Boolean circuit model, called $n$-wire local railway circuits, where $n$ parallel wires are straddled by Boolean gates, each with matching fanin/fanout strictly less than $n$, and we show that such a model can not count to $2^n$ nor implement any so-called odd bijective nor quasi-bijective function. We then define a class of self-assembly systems that includes theoretically interesting and experimentally-implemented systems that compute $n$-bit functions and count layer-by-layer. We apply our Boolean circuit result to show that those self-assembly systems can not count to $2^n$. This explains why the experimentally implemented iterated Boolean circuit model of tile assembly can not count to $2^n$, yet some previously studied tile system do. Our work points the way to understanding the kinds of features required from self-assembly and Boolean circuits to implement maximal counters.

==> app-sa.tex <==
%auto-ignore
\section{Self-assembly: iterated layers}\label{sec:app:iterated layers}

% !TEX root = cpibc-main.tex

\begin{definition}[Computing an iterated $n$-bit function]\label{def:assemble an iterated layer function}
The tile set $T$ is said to layer-compute $f^k$, 
i.e., $k$ iterations of the Boolean function $f : \{0,1\}^n\rightarrow\{0,1\}^n$,  
 if 
\begin{enumerate}[(a)]
\item $T$ layer-computes $f$ via Definition~\ref{def:assemble a layer function}, and 
\item $\calT_x$'s terminal assembly $\alpha_x$, for each $i\in \{0,1,\ldots,k-1\}$, has
$\calB(\gac{ \alpha_x}{(c + i \cdot \vec v)}) = f^i(x)$.
%\footnote{We use the notation $f^i$ to mean the $i^\textrm{th}$ composition of $f$.}
\end{enumerate}
\end{definition}
\begin{lemma}\label{lem:self-assembly of a layer fn}
Let $T$ be a tile set that  layer-computes the $n$-bit function $f$ %$f : \{0,1\}^n\rightarrow\{0,1\}^n$ 
according to Definition~\ref{def:assemble a layer function}. 
Then for any $k\in\Nset$, $T$ also computes 
$f^k$ according to Definition~\ref{def:assemble an iterated layer function}.
\end{lemma}
\begin{proof} 
We give a simple proof by induction on iteration $f^i$ for $i \in \{0,1,\ldots,k-1 \} $. 
The intuition is to let $y' = f^i(x) \in \{0,1\}^n$, then use Definition~\ref{def:assemble a layer function} 
to compute $f^1(y')$, and then translate the resulting assembly to a later layer to compute $f^{i+1}(y') = f( f^{i}(y') )$.

For the base case, let $i=0$. By Definition~\ref{def:assemble a layer function}, the seed $\sigma_x$ encodes $x\in\{ 0,1\}^n$ along $c$ as $\calB(\gac{\sigma_x}{c})=x$ and $\sigma_x$ places no tiles in $\mathrm{RHS}(c) \subsetneq \Zset^2$. 
Hence $T$ computes $f^0(x)=x$ according to Definition~\ref{def:assemble an iterated layer function}.

For the inductive case, let $i > 0$.
Let $\vec{\alpha} = \alpha_0,\alpha_1,\ldots,\alpha_m$ be an assembly sequence of $\calT_x$ such that, inductively, we assume that on the last assembly $\alpha_m$ of $\vec\alpha$ the cut $c + i \cdot \vec v$ encodes the bit sequence 
%$y' = \underbrace{f(f(\ldots f(x))}_{i \text{ times}} \in \{0, 1\}^n$, 
% $y' = f^i(x) \in \{0, 1\}^n$ as 
$f^i(x) = \calB(\gac{\alpha_x}{(c+\vec i \cdot v)}) \in \{0, 1\}^n$, 
and $\alpha_m$ has no tiles in $\mathrm{RHS}(c + i \cdot \vec v)$, and 
no more tiles can stick in $\mathrm{LHS}(c + i \cdot \vec v)$.
Next, consider the seed assembly $\sigma_{y'}$ that encodes $y' = f^i(x)$, and let 
$\vec{\alpha} = \sigma_{y'}, \alpha_1, \alpha_2, \ldots $ 
be an assembly sequence that satisfies   
Definition~\ref{def:assemble a layer function}(\ref{def:condition:niceseq}) and (\ref{def:condition:tile placements map to gate}).
For each $k \in \{ 0, 1,\ldots, |\vec{\alpha} |-1 \}$ 
%assembly $\alpha_k$ of the assembly sequence $\vec{\alpha}_{y'}$ in order, 
let $(t,z)_k$ be the tile that sticks (is attached) to assembly 
$\alpha_k$ to give the next assembly $\alpha_{k+1}$ in~$\vec\alpha$. 
% Consider the translated tile 
We make a new assembly sequence $\vec{\alpha}'$
that starts with the assembly $\alpha_m$ (defined above), 
then stick the `translated tile' 
$(t,z + i\cdot \vec v)_0$, 
and then sticks $(t,z + i\cdot \vec v)_1$, and so on.
  In other words define
  $\vec{\alpha}' = \alpha_{m,0} \rightarrow_\calT \alpha_{m,1} \rightarrow_\calT \cdots $ by beginning with 
  $ \alpha_{m} = \alpha_{m,0}$ and in turn attaching the tiles 
$(t,z + i\cdot \vec v)_0, (t,z + i\cdot \vec v)_1,\ldots $
 in order. 
 the assembly sequence 
$\vec{\alpha}'$ 
eventually contains an assembly that encodes $f(y') = f^{i+1}(x)$ along the curve $c + (i+1)\cdot \vec v$ as $f^{i+1}(x) = \calB(\gac{\alpha_x}{(c+ (i+1)\cdot\vec v)})$. 
This completes the induction.
\end{proof}



==> app-zigzag_figure.tex <==
%auto-ignore
% !TEX root = cpibc-main.tex

\section{Zig-zag Figure}\label{sec:app-zigzag_figure}
\begin{figure}[h]
\includegraphics[width=\textwidth]{images/zigzag}
\caption{Zig-zag tile assembly system, similar to Evans~\cite{evans2014crystals}. (a)~Schematic of a zig-zag system showing the seed $\sigma_x$ and arrows indicating tile attachment order. 
The first column of tiles (``zig'') implements a binary increment, using tile types similar to those in Figure~\ref{fig:zigzig}(a),
the second column of tiles (``zag'')  copies a columns of input bits to the right.    
The choices for the curve $c$ (in green) and vector $\vec v = (2,0)$ for Definition~\ref{def:assemble a layer function} are shown. 
(b)~A layer consists of a single zig (tiles at positions $z_0,\ldots,z_5$) followed by a zag (tiles at position $z_6,\ldots,z_{11}$,). 
Intuitively, because some glues output constant bits (e.g. $x_0=y_0=1$ we are free to choose whether 
those glues should be 0/1-encoding glues (black), and $\epsilon$-glues (grey), in (b) we have all glues be 
0/1-encoding which leads to a valid 
railway circuit in (c) that simulates the tile layer in (b).
Specifically, in (c) all gates having fanin and fanout that is equal; in other words the functions 
from one green/blue cut to the next green/blue cut are all from $n$ bits to $n$ bits.
Moreover, no gate spans all 6 wires hence the railway circuit is local.
Hence our main theorem applies that this system does not implement a $2^n$ counter on $n=6$ bits (it does however, implement a $2^{n-1}$-counter on $n=6$ bits).
(d)~If we instead assume that $x_0, y_0$ are $\epsilon$-glues, we get a maximal $2^n$ counter (but on only $n=5$ bits). 
In (e) the resulting circuit is not a railway circuit since some gates $z_0, z_4, z_6, z_{10}$ have unequal fanin and fanout.
Unequal fanin and fanout means that the function from blue/green cut to blue/green cut are not all on a fixed number $n$ bits, hence our techniques do not apply. 
}\label{fig:zigzag}
\end{figure}


==> circuit_definitions.tex <==
%auto-ignore
% !TEX root = cpibc-main.tex

\newcommand{\ORgate}{\textsc{Or}}
\newcommand{\ANDgate}{\textsc{And}}
\newcommand{\NOTgate}{\textsc{Not}}
\newcommand{\XORgate}{\textsc{Xor}}
%\newcommand{\ORACLEgate}{\textsc{Oracle}}

\newclass{\DLOGTIME}{DLOGTIME}
\newclass{\FL}{FL}
\newclass{\FAC}{FAC}
\newclass{\FNC}{FNC}
\newclass{\tally}{tally}
\newclass{\COR}{OR}
\newclass{\CAND}{AND}
\newclass{\CANDCOR}{\CAND\textrm{-}\COR}

\newlang{\Parity}{Parity}



\newcommand{\Reducible}[3]{\ensuremath{#2_{\mathrm{#1}}(#3)}}


\newcommand{\bigO}[1] {\ensuremath{\mathcal{O}(#1)}}
\newcommand{\nats}{\ensuremath{\mathbb{N}}}
\newcommand{\tallyMachine}{\ensuremath{\mathcal{M}}}

\newcommand{\semiencoder}{\ensuremath{h}}
\newcommand{\former}{\ensuremath{f}}

\newcommand{\uniform}      [2]{\ensuremath{#1\textrm{-uniform-}#2}}
\newcommand{\semiunif}      [2]{\ensuremath{#1\textrm{-semi-uniform-}#2}}
\newcommand{\uniformAND}    [1]{\ensuremath{#1\textrm{-uniform-}\CAND}}
\newcommand{\uniformOR}    [1]{\ensuremath{#1\textrm{-uniform-}\COR}}
\newcommand{\semiuniformOR}[1]{\ensuremath{#1\textrm{-semi-uniform-}\COR}}
\newcommand{\semiuniformAND}[1]{\ensuremath{#1\textrm{-semi-uniform-}\CAND}}
\newcommand{\FOSOR}{\ensuremath{\semiuniformOR{\FAC^0}}}  
\newcommand{\FOSAND}{\ensuremath{\semiuniformAND{\FAC^0}}}  
\newcommand{\FOOR}{\ensuremath{\uniformOR{\FAC^0}}} 
\newcommand{\FOAND}{\ensuremath{\uniformAND{\FAC^0}}} 



  \section{Boolean circuit definitions}
  \label{sec:defs}
  We now give some basic  definitions based on those in the
  literature~\cite{AK2010, AJ1993, GHR1995x}.  For more details
  on Boolean circuits see~\cite{Vol1999x}.


  For a function $f \colon \{0,1\}^* \to \{0,1\}^*$ and integer $n \geq 1$
  let $f_n \colon \{0,1\}^n \to \{ 0,1\}^{n}$ be the restriction of $f$ to
  domain and range consisting of strings of length $n$ respectively. 
  
  An \emph{iterated circuit layer} on $n$ variables $w_0,\ldots,w_{n-1}$ is a directed acyclic
  graph. 
  each vertex of the circuit is defined to be one of  gate, input or output. 
  Inputs have in-degree 0 and arbitrary out-degree,   
  outputs have arbitrary in-degree and out-degree-0, and 
  gates have arbitrary in- and out-degree. 
 The iterated circuit layer has $n$ inputs labelled $x_0,x_1,\ldots x_{n-1}$ and $n$ outputs labelled $y_0,y_1,\ldots y_{n-1}$. 
  % The in-degree (out-degree) of a gate is called its fan-in (fan-out).  Each source vertex
%  (fan-in 0) is labelled either by one of the input variables $w_0,\ldots,w_{n-1}$ or by a constant ``0'' or ``1'' (false or true).  
Each non-source vertex is labelled by a function name, such as $\ANDgate$,
  $\ORgate$, $\NOTgate$, $\XORgate$, etc. 
  Gates with fan-out of 0 (called sinks) are permitted, as are gate of fan-in 0 (called constant-0 or constant-1 gates). 
  
  Given an input $x \in \{0, 1\}^n$, one can inductively assign a Boolean value
  to each vertex of an iterated circuit layer as follows: each input vertex gets the value of that variable, each constant vertex labelled by a constant gets the value of that constant,
  and each other vertex gets the value of the function that labels it applied to
  the values of its children. 
  
\dw{TODO:}  An iterated circuit is defined as ... circuit inputs, paste together circuit layers (input of layer $i$ are  identified with outputs of layer $i-1$)....
  
  Notion of ``cut $i$'' of the circuit being the sequence of $n$ output values of layer $i$ ...
 
 
  
  \dw{Probably not needed in this paper:}
 The \emph{depth} of a circuit is the length of the longest path from an input vertex to an output vertex. 
The \emph{size} of a circuit is the number of wires it contains~\cite{AK2010}.
%  A circuit computes a function on a fixed number of Boolean variables.  We
%  consider functions of an arbitrary  number of variables by defining (possibly
%  infinite) families of circuits.  We say a family of circuits~$\mathcal{C} =
%  \{ C_n \mid n \in \mathbb{N} \}$ computes a function~$f \colon \{0, 1\}^* \to
%  \{0, 1\}^*$ if for all $n \in \mathbb{N}$, and for all $w\in\{ 0,1\}^n$
%  circuit  $C_n$ outputs the string $f(w)$ (we consider only functions $f$
%  where for each $n$ there is an $m$ where all length-$n$ strings in $f$'s
%  domain are mapped to length-$m$ strings).  We say a family of circuits
%  $\mathcal{C}$ decides a language~$L \subseteq \{ 0,1\}^*$ if for each~$w\in\{0,1\}^n$ circuit~$C_n
%  \in \mathcal{C}$ on input $w$ outputs~$1$ if~$w \in L$ and~$0$ if~$w \notin
%  L$.
  
  
%  
%  \vspace{30ex}
%  {\bf DW: THE REST IS PROBABLY NOT NEEDED }\\
%  In a \emph{non-uniform} family of circuits there is no required  
%   similarity between family members.    
%  In order to specify such a requirement   
%  we use a {\em uniformity function} that 
%  algorithmically specifies the similarity between members of a circuit family. 
%  Roughly speaking, a \emph{uniform circuit family}~$\mathcal{C}$ is an infinite sequence of
%  circuits with an associated function~$\former : \{1\}^* \rightarrow
%  \mathcal{C}$ that generates members of the family and is
%  computable within some resource bound.  
% More precisely:  
%
%
%  \begin{definition}[$\C$-Uniform circuit family]
%    Let $\C$ be a set of functions. A circuit family $\mathcal{C}$ is
%    $\C$-uniform, if there is function $f \in \C$, $\former : \{1\}^* \rightarrow
%  \mathcal{C}$, where $f(1^n) = C_n$ for all $n \in \mathbb{N}$, 
%  and $C_n \in  \mathcal{C}$ is a description of
%  a circuit with $n$ input gates (we use $C_n$ to denote
%  either a circuit or its encoding as a binary string).
%  \end{definition}
%
%  When dealing with uniformity for small complexity classes one of the more 
%  preferred uniformity conditions is $\DLOGTIME$-uniformity~\cite{BIS1990p}.
%  This definition uses a unique ordering on wires that leave and enter a given gate.
%  
%  \begin{definition}[\cite{AK2010}]
%    \label{def:dlogtime}
%    A circuit family $\mathcal{C}$ is $\DLOGTIME$-uniform if there is
%    a procedure that on input $(n, i, r, j, s, t)$, where $n, i, r, j,  s \in
%    \mathbb{N}$ are encoded in binary and $t$ is a gate type (e.g., $\ANDgate$,
%    $\ORgate$, $\NOTgate$,  input, 0, 1) encoded in binary, runs in time
%    \emph{linear} in its input size and accepts if and only if the gate of
%    $C_n$ having label $i$ is of type~$t$ and its $r$-th child is the $s$-th
%    output  of the gate having label $j$.  In the case where gate $i$ is an input
%    gate, the procedure accepts if gate $i$ takes the value of the $s$-th input
%    bit.  Furthermore, the procedure accepts inputs of the form $(n, i, j, s,
%    output)$ if and only if the $s$-th output wire of gate $i$ is the $j$-th
%    output gate 
%    of the circuit $C_n$.  We also require that the procedure
%    accepts the input $(n, i, d)$ if and only if $d$ is equal to the fan-in of
%    the gate of $C_n$ having label $i$. 
%  \end{definition}
%  
%  $\AC^0$ is the set of languages decidable by constant-depth polynomial-size
%    (in input length~$n$) $\DLOGTIME$-uniform circuits built using unbounded
%    fan-in $\ANDgate$ and $\ORgate$ gates, and $\NOTgate$ gates with fan-in 1.
%  $\FAC^0$ is the class of functions computable by polynomial-size
%    constant-depth $\DLOGTIME$-uniform circuits built using unbounded fan-in
%    $\ANDgate$ and $\ORgate$ gates, and $\NOTgate$ gates with fan-in 1.
%
%  An \emph{$\ORgate$ circuit} is a circuit that uses only disjunctive
%  logic, that is, a circuit that has only $\ORgate$, constant, and input
%  gates. One of the $\ORgate$ gates is denoted as the output gate.
%  Similarly an \emph{$\ANDgate$ circuit} is a circuit that uses only conjunctive
%  logic, that is, a circuit that has only $\ANDgate$, constant, and input
%  gates. One of the $\ANDgate$ gates is denoted as the output gate.
%  Note that $\ORgate$  and $\ANDgate$ circuits may have multiple non-output sinks.
%    Let non-uniform-$\COR$ (non-uniform-$\CAND$) be the set of decision problems that solved by non-uniform families of
%  $\ORgate$ ($\ANDgate$) circuits.
%  
%  In this paper, we are concerned with $\FOOR$: the class of languages solved
%  by uniform polynomial size  $\ORgate$ circuits, formally defined as follows.
%  \begin{definition}
%    Let $\FOOR$ be the set of decision problems over the 
%    alphabet $\{ 0,1\}$ that are solved by $\FAC^0$ uniform families of $\ORgate$ 
%    circuits. 
%  \end{definition}
%  The class $\FOAND$ is defined analogously, but using $\ANDgate$ instead of $\ORgate$ circuits.
%  \begin{lemma}
%    \label{lem:OR_noteq_AND}
%    $\uniformOR{\FAC^0} \neq \uniformAND{\FAC^0}$.
%  \end{lemma}
%  \begin{proof} 
%    An $\ORgate$ circuit computes an $\ORgate$ function on some subset of its
%    inputs; in general there is no $\ANDgate$ circuit that computes the same function, and
%    vice-versa.  
%  \end{proof}
%
%  $\NL$ is the class of languages accepted  
%  by non-deterministic logarithmic-space Turing machines. Such machines have a 
%  read-only input tape, a write-only output tape and a read-write work tape 
%  whose length is a logarithmic function of  input length. 
%  The class of functions $f: \{0,1\}^* \to \{0,1\}^*$
%  computed by non-deterministic logarithmic-space Turing machines (with an
%  additional write-only output tape) is denoted $\FNL$.
%  Let $\tally$ be the set of all languages over the one-letter alphabet $\{ 1\}$.
%  We define  $\tally\NL = \tally \cap \NL$, i.e.\ the class of all tally
%  languages in $\NL$.  
%  Let $\tally\co\NL = \tally \cap \co\NL$.
%  The following lemma follows from $\NL = \co\NL$,
%    (i.e.\ let $L \in \tally\NL \subsetneq \NL = \co\NL$,
%    then $L \in \co\NL$ implies $L \in \tally\co\NL$;
%    a similar argument holds for the converse):
%  \begin{lemma}
%    \label{lem:tallynl_eq_tallyconl}
%    $\tally\NL = \tally\co\NL$
%  \end{lemma}
%  We also make use of
%  functions from the class $\tally\FAC^0 = \tally \cap \FAC^0$ which is
%  contained in $\tally\NL$.
%  
%  Each language $L \subseteq
%  \{ 0,1\}^{\ast}$ has an associated total \emph{characteristic function}
%  $\chi_L \colon \{ 0,1\}^{\ast} \to \{0, 1\}$ defined  by $\chi_L (w) = 1$
%  if and only if $w \in L$.  
%      
%  $\Parity \subseteq \{ 0,1\}^*$ is the set of binary strings that contain an odd number of 1s.
%
%  
%    \subsection{Reductions} 
%    For concreteness, we explicitly define some standard types of reductions. 
%    Let $A, B \subseteq \{ 0,1\}^{\ast}$.
%  
%    \begin{definition}[Many-one reducible]
%      \label{def:many_One_reduction}
%      Set $A$ is many-one reducible to set $B$, written $A \leq^{\C}_m B$,
%      if there is a function $f$ that  is $\C$-computable with the
%      property that for all $w$, $w \in A$, if and only if $f(w) \in B$.
%    \end{definition}
%
%    The following definition of truth table reductions comes
%    from~\cite{BB1988,BHL1995}, for a more formal definition see~\cite{LLS1975}.
%  
%    \begin{definition}[Truth-table reduction]
%      \label{def:truthtablereduction}
%      Set $A$ is $\C$ truth-table reducible to $B$,
%      written $A \leq^{\C}_{tt}B$,
%      if there exists $\C$-computable functions $\tau$
%        and $\sigma$ 
%        such that for all $w \in \{0,1\}^*$,
%        $\tau(w)$ is 
%          a list of $\ell \in \mathbb{N}$ strings $ a_1, \ldots, a_{\ell}$,
%        also $\sigma(w)$ is a truth table (Boolean function) with $\ell$ variables,
%        and $w \in A$ if and only if 
%        $\sigma( \chi_B(a_1),\ldots, \chi_B(a_{\ell}) )$ evaluates to true,
%        where
%        $\chi_{B}$ is the characteristic function of $B$.
%    \end{definition}
%    A \emph{disjunctive} truth table reduction (dtt) is one where 
%      at least one string generated by $\tau(w)$ is in~$B$.
%    Or equivalently, where $\sigma(w) = \bigvee_{1\leq i \leq \ell} \chi_B(a_i)$.
%    A \emph{conjunctive} truth table reduction (ctt) is one where 
%      all the strings generated by $\tau(w)$ are in $B$.
%    Or equivalently, where $\sigma(w) = \bigwedge_{1\leq i \leq \ell} \chi_B(a_i)$.
%
%    \begin{definition}[Turing reducible]
%      \label{def:turing_reduction}
%      Set $A$ is $\C$ Turing reducible to $B$, written $A \leq^{\C}_{T}B$, if
%      there is a $\C$-computable oracle circuit (or Turing machine) $M$ such that   $w \in A$
%      iff $M$ accepts $w$ with $B$ as its oracle. 
%    \end{definition}
%
%    The following implications follow directly from these definitions, 
%      for more details see~\cite{LLS1975}.
%      \begin{equation*}
%        \begin{tikzpicture}[baseline]
%          \matrix (m) [row sep=-1em, column sep=-0.8em]{
%            & \node[rotate=15]{$\implies$}; & \node{$A \leq^{\C}_{dtt} B$}; & \node[rotate=-15]{$\implies$}; & \\ 
%             \node{$A \leq^{\C}_{m} B$}; & & & & \node{$A \leq^{\C}_{tt} B \implies A \leq^{\C}_T B$ };\\ 
%            & \node[rotate=-15]{$\implies$}; & \node{$A \leq^{\C}_{ctt} B$}; & \node[rotate=15]{$\implies$}; & \\
%          };
%        \end{tikzpicture}
%      \end{equation*}
%  
%    Let $\Reducible{r}{\FAC^0}{\C}$ be the set of all languages that are
%      $\FAC^0$ reducible to languages in $\C$ via some type of reduction 
%      $\mathrm{r} \in \{ \text{m, dtt, ctt, tt, T} \}$. 
%
%  \subsection{Some useful $\FAC^0$ functions}
%    \label{sec:facfunc}
%    \paragraph{Pairing function}
%    We require a pairing function that is injective and extremely easy
%    ($\FAC^0$) to compute.  We use the pairing function
%    that interleaves the bits of two binary string arguments $a$ and $b$. For
%    example, the binary strings $a=a_2 a_1 a_0$ and $b=b_2 b_1 b_0$ are paired
%    as the interleaved string $\langle a,b \rangle =
%    b_2 a_2 b_1 a_1 b_0 a_0$.
%    The circuits for interleaving and de-interleaving have only  a single input gate layer and
%    a single output gate layer (and so are 2-layer $\AC^0$ circuits). This circuit can be shown to be
%    $\DLOGTIME$-uniform.   
%
%    \paragraph{Binary to Unary}
%    There is a 
%      constant depth
%        circuit family where circuit $C_n$ 
%        takes as input some word  $w\in \{0,1\}^n$ 
%        and outputs $1^x$ where $x$ is the positive integer encoded in the 
%        first $\lceil\log_2 n \rceil$ bits of $w$~\cite{CSV1984}. 
%    It can be shown that this circuit family is  
%      $\DLOGTIME$ uniform and so this conversion from short binary strings to unary is in $\FAC^0$. 
%
%    \paragraph{Unary to Binary}
%    There is a 
%      constant depth
%        circuit family where circuit $C_n$ 
%        takes as input some word $w = 0^{n-x} 1^x$ where $0 \leq x \leq n $,
%        and outputs the binary encoding of $x$~\cite{CSV1984}. 
%    It can be shown that this circuit family is $\DLOGTIME$ uniform and so 
%      unary to binary conversion is in $\FAC^0$.
% 
%    \subsection{Configuration graphs}
%    \label{sec:config_graphs}
%    \begin{definition}[Configuration Graph]
%     Let $w \in \{0,1\}^*$ be the input to a halting Turing machine~$M$. 
%      The \emph{configuration graph} $C_{M,w}$ is a directed acyclic graph 
%        where each vertex encodes a configuration of $M$ 
%        on inputs of length $|w|$.         
%      The graph $C_{M,w}$ has a directed
%          edge from a vertex~$c$ to a vertex $c'$ if the configuration encoded by $c'$ 
%          can be reached from the configuration encoded by~$c$ in one
%          step via $M$'s transition function.
%    \end{definition}
%
%    
%    A configuration graph $C_{M,w}$ has the property that there is a directed
%      path from the vertex $c_s$ representing the start configuration, to the accept vertex $c_a$ 
%      if an only if $M$ accepts input~$w$. 
%    Lemma~\ref{lem:config_in_AC0} follows from~\cite{Imm1987,Imm1999x}. 
%      
%      
%      
%      
%    
%      
%      
%
%      
%      
%      
%    \begin{lemma}
%      \label{lem:config_in_AC0}
%      Given the binary encoding of 
%        a Turing machine $M$, which has state set $Q$ and
%        has an $\FAC^0$ computable space bound $s = \bigO{\log |w|}$,
%        and given an input $w$, 
%        the configuration graph $C_{M,w}$  
%        is computable in $\uniform{\DLOGTIME}{\FAC^0}$
%        and is  of size $\bigO{2^s |w| |Q|}$.
%    \end{lemma}


==> proof_christopher.tex <==
%auto-ignore
Denote $f\colon X \to Y$ a map between any pair of sets.

Define :
$degRam_y(f) = \left( \#f^{-1}(y) - 1 \right)^+$ which is the number of antecedants minus one if $y$ in the image and $0$ if not.
$totRam = \sum_Y degRam_y(f)$ the total ramification degree.

Lemma : $totRam(f) = \# X - \# \left( X/\sim_f \right)$ where $X/\sim_f$ is the quotient of $X$ by the relation $x\sim x' \iff f(x)=f(x')$, thus $f$ partitions $X$ by the sets $f^{-1}(y)$ with equal values, and the total ramification degree substracts the nuhmber of parts to the maximum number of parts imaginable, in particular it is inversely proportional to the number of parts.

Now let $f\colon X \to Y$ and $g\colon Y \to Z$ be maps with possibly infinite total ramification totRam(f) and totRam(g).

Lemma : $totRam(gf)\geq \max(totRam(f),totRam(g))$.

Proof : We wish to show that $\# X/ \sim_{fg} \leq \# X/ \sim_{f}$ and $\# X/ \sim_{fg} \leq \# X/ \sim_{g}$, but the secnod is obvious and the first follows from the fact that the relation $\sim_{gf}$ is a quotient of $\sim_f$. Indeed, denoting $\tilde{f} \colon X/\sim_f \to Y$ the injection one has $X/\sim_{fg} = (X/\sim_{f})/\sim_{g \tilde{f}}$.

==> self_assembly__2020_4_30.tex <==
%auto-ignore
% !TEX root = cpibc-main.tex

\newcommand{\calT}{\mathcal{T}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\Nset}{\mathbb{N}}
\newcommand{\Zset}{\mathbb{Z}}
\newcommand{\Hset}{\mathbb{H}}
\newcommand{\Rset}{\mathbb{R}}
\newcommand{\CS}{\mathrm{CS}}


\newpage
\section{Self-assembled counters}

Here we apply the  Boolean circuit framework already established in previous sections to show limitations of self-assembled counters that work in base 2.

\subsection{Self-assembly: Definitions}

We give a short definition of the abstract Tile Assembly Model (aTAM)~\cite{Winf98,DotCACM} here, more details can be found elsewhere~\cite{PatitzSurveyJournal}.

% A tile type, is a square tile, with each side having an associated  glue (taken from a finite set of glues types $G$), and natural number strength.  
% Let $b\in\mathbb{N}$, $b \geq 2$, be called the {\em base}. 
In the aTAM, one considers a set of square tile types $T$ where each square side has an associated {\em glue type}, a pair $(g,s)$  where $g$ is a (typically binary) string and $s \in \mathbb{N}$ is a glue strength. 
We let $G$ denote the of all glue types of $T$. 
A tile $(t,z) \in T\times\Zset^2$ is a positioning of a tile type on the integer lattice. 
A glue is a pair $(g,z) \in G\times \Hset$ where 
$\Hset$ is the set of half-integer points $\Hset = \left\{ z \pm h \mid z \in \mathbb{Z}^2 , h \in  \{ (0,0.5) , (0.5,0) \} \right\}$.
%We consider the notion that each glue has an interpretation as a bit (or {\em counter-symbol}) via the function 
%$\CS : G\times \Hset \rightarrow \{0,1\}$. 
We consider the notion that each glue type has an interpretation as a bit (or {\em counter-symbol}) via the function 
$\CS : G\rightarrow  \{0,1\}$. 

An assembly is a partial function $\alpha : \mathbb{Z}^2 \rightarrow T$, whose domain is a connected set. 
For $X\subset\Zset^2$ we let $\alpha |_X$ denote the restriction of $\alpha$ to domain $X$, i.e.\ $\alpha |_X : X\rightarrow T$ and for all $z\in X$, $\alpha(z)=\alpha |_X(z)$. 


Let $\mathcal{T} = (T,\sigma,\tau)$ be an aTAM system where
$T$ is a set of tile types, $\tau \in \mathbb{N}^+$ is  the temperature and $\sigma$ is an assembly called the seed assembly. 
% A {\em tile} is a pair $(t,z)$ where $t$ is a tile type and $z\in\Zset$. 
%Starting from the seed assembly, intuitively, tiles are added one at a time to a growing assembly. 
The process of self-assembly proceeds as follows.
A tile $(t,z)$ {\em sticks} to an assembly $\alpha$ if $z\in\Zset^2$ is adjacent in $\Zset^2$ to (but not on) a tile position of $\alpha$ and the glues of $t$ that touch\footnote{A pair of glues touch if they share the same half-integer position in $\Hset$.} glues of $\alpha$ of the same glue type have the sum of their strengths being at least $\tau$. 
The resulting new assembly $\alpha'= \alpha\cup \{ z\rightarrow t \}$ is said to contain the tile $(t,z)$, and we write $\alpha \rightarrow_\calT \alpha'$. 
In an {\em  assembly sequence} $\vec \alpha = \alpha_0, \alpha_1 \ldots, \alpha_k$,  for each assembly one tile sticks to the previous assembly: $
\alpha_0 \rightarrow_\calT \alpha_1 \rightarrow_\calT \cdots \rightarrow_\calT \alpha_k$.
A terminal assembly of $\calT$ is an assembly to which no tiles stick. 
$\calT$ is said to be {\em directed} if it has exactly one terminal assembly and undirected otherwise.


\subsection{Self-assembling Boolean layer functions}

\begin{definition}[glue curve]
A {\em glue curve} $c : (0,1)\rightarrow\Rset^2$ is an infinite simple curve\footnote{A simple curve is a mapping from the open unit interval $(0,1)$ to $\Rset^2$ that is non-self-intersecting.}
that starts as of an infinite vertical ray from the south, then has a finite number of unit-length straight-line glue segments that each touch a single point in $\Hset$, and ends with an infinite vertical ray to the north.
\end{definition}
By a generalisation of the Jordan curve theorem to infinite polygonal curves (see, for example, Theorem~B.3 in~\cite{paths2020}), $c$ cuts the $\Rset^2$ plane in two, and hence we let $\mathrm{LHS}(c) \subsetneq \mathbb{Z}^2$ denote the points of  $\mathbb{Z}^2$ that are on the left-hand side\footnote{Intuitively, the left-hand side of a glue curve (or any an infinite simple curve) is the set of points from $\Rset^2$ that are on one's left-hand side as one walks along the curve, excluding the curve itself. See~\cite{paths2020} for a more formal definition appropriate to glue curves.} of $c$, and 
$\mathrm{RHS}(c) \subsetneq \mathbb{Z}^2$ denote the points of  $\mathbb{Z}^2$ that are on the right-hand side of $c$.
For a vector $\vec v$ in $\Rset^2$ we define 
$c + \vec v$ to be the curve 
$\cup_{x\in (0,1)}  c(x)+\vec v$ 
i.e. the translation of the range of $c$ by $\vec v$. 

%\begin{definition}[Encoding of a bit string along a curve]\label{def:bit encoding}
%Let $n \in \Nset$, and $c$ be a glue curve. 
%We say that the function $\mathcal{G}_c$ encodes a bitstring along the curve $c$ if $\mathcal{G}_c$ is a bijective function 
%that maps each n-bit sequence to a sequence of $\geq n$  glues positioned along $c$, formally: $\mathcal{G}_c : \{ 0,1\}^n \rightarrow \cup_{m \geq n} \{ G \times  (\Hset \cap \mathrm{range}(c)) \}^{m}$. 
%\dw{... and this function is somehow consistent with applying $\CS$ ... but $\mathcal{G}$ may use several glues to represent one bit ...maybe change 
%$m$ to $n$.}
%\end{definition}
%
%We call $\mathcal{G}_c$ the glue encoding function,  and it's inverse, $\mathcal{G}_c^{-1}$, the glue decoding function.


\begin{definition}[Encoding of a bit string along a curve]\label{def:bit encoding}
Let $n \in \Nset$, and $c$ be a glue curve. 
We say that the function $\mathcal{G}_c$ encodes a bitstring along the curve $c$ if $\mathcal{G}_c$ is a bijective function 
that maps each n-bit sequence to a sequence of $\geq n$  glues positioned along $c$, formally: $\mathcal{G}_c : \{ 0,1\}^n \rightarrow \cup_{m \geq n} \{ G \times  (\Hset \cap \mathrm{range}(c)) \}^{m}$. 
\dw{... and this function is somehow consistent with applying $\CS$ ... but $\mathcal{G}$ may use several glues to represent one bit ...maybe change 
$m$ to $n$.}
\end{definition}

We call $\mathcal{G}_c$ the glue encoding function,  and it's inverse, $\mathcal{G}_c^{-1}$, the glue decoding function.


\begin{definition}[Layer-computing an $n$-bit layer function]\label{def:assemble a layer function}
The tile set $T$ is said to layer-compute the Boolean function $f : \{0,1\}^n\rightarrow\{0,1\}^n$  
if there exists  
a temperature $\tau\in\Nset$,
a glue curve $c$, 
a glue encoding function $\mathcal{G}_c$,
and a vector $\vec v$ with positive $\mathrm{x}$-component such that, 
for all $i > 1$, $c \cap (c+i\cdot v) = \emptyset$, 
and for all $x \in \{0,1\}^n$
there is an assembly $\sigma_x$ on the left-hand side of $c$, 
such that the tile assembly system $\calT_x = (T,\sigma_x,\tau)$  is directed and the following hold: 
\begin{enumerate}[(a)]
%\item $\sigma_x$ encodes $x$ along $c$, $\sigma_x|_{\mathrm{LHS}(c)} = \sigma_x$, 
\item $\mathcal{G}_c(x)$ defines the glues of $\sigma_x$ that are on $c$, 
\item $\calT_x$'s terminal assembly $\alpha_x$ has the glues $\mathcal{G}_c(f(x))$ on the curve $c + \vec v$,
 
\item\label{def:condition:niceseq} $\calT_x$ has at least one assembly sequence that assembles all of $\alpha |_{\mathrm{LHS}(c + \vec v)}$ before placing any tile of 
$\alpha |_{\mathrm{RHS}(c + \vec v)}$. 
% ``$\alpha$ restricted to LHS $c + \vec v$'' before placing a tile to the right of $c + \vec v$. 
\end{enumerate}
\end{definition}

\dw{in the previous def, do we need to say anything about how ``signals'' are propagated through the assembly (for proof of final lemma)?}

\newpage

\begin{definition}[Self-assembling an iterated $n$-bit layer function]\label{def:assemble an iterated layer function}
The tile set $T$ is said to compute
% $$ \underbrace{f(f(\ldots f(x))}_{k \text{ times}} = y \in \{0, 1\}^n$$ 
 $k$ iterations of the Boolean function $f : \{0,1\}^n\rightarrow\{0,1\}^n$    if 
\begin{enumerate}[(a)]
\item $T$ layer-computes $f$ via Definition~\ref{def:assemble a layer function}, and 
%using temperature $\tau$, curve $c$, vector $\vec v$ and glue encoding function $\mathcal{G}_c$, and 
\item $\calT_x$'s terminal assembly $\alpha_x$, for each $i\in \{0,1,\ldots,k-1\}$, encodes $\mathcal{G}_{c + i \cdot \vec v}(f^i(x))$ 
 along the glue curve $c + i \cdot \vec v$.\footnote{We use the notation $f^i$ to mean the $i^\textrm{th}$ composition of $f$.}
% $T$ also computes the $k$th iteration of~$f$  in the sense that the terminal assembly of $\calT_x$ encodes $y$ along the glue curve $c + k \cdot \vec v$.
\end{enumerate}
\end{definition}

\subsection{Self-assembly: Positive results to illustrate the setup}
The results in this subsection are not necessary to prove our main result on self-assembly (Theorem~\ref{thm:self-assembly:no max counter}), but are here to (a) illustrate the previous definitions and (b) show they are reasonable since they encapsulate previously studied systems. 



\begin{figure}
\includegraphics[width=\textwidth]{images/counters_cuts}
\caption{
Limitations of self-assembled counters. 
Left: First few layers of a 6-bit 63-counter for the 6-bit IBC tile model that appeared in~\cite{WoodsDotyWinfree}.
Theorem~\ref{thm:self-assembly:no max counter}, shows that although there are 64 possible bit-strings that appear across the all cuts for all 6-bit systems, no 64-counter is possible in any one system. 
The layers here are of depth one ($\vec v$ is such that layers are one tile deep ... ). 
Our result would still hold even if the layers were of {\em any} constant depth.
The cuts $c$ and $c+\vec v$ used in  Definition~\ref{def:assemble a layer function}, 
as well as subsequent cuts used in Lemma~\ref{lem:self-assembly of a layer fn}, 
are shown in green. 
The lattice is rotated by $45^\circ$, relative to the standard $\Zset^2$ lattice. 
Right: An Evans-Winfree counter~\cite{evans2014crystals}. In this kind of counter uses base 4 (glues) to count in base 2 to $2^n$. Our result shows that in this setting have base strictly greater than 2 is required. In other words, there is no base 2 $2^n$-counter in the aTAM. 
\dw{TODO How to handle null glues?}
}
\end{figure}

\begin{example}
\dw{Here or after the next lemma, insert some examples from the literature. show that our defs admit those known examples.}
\end{example}

\begin{lemma}\label{lem:self-assembly of a layer fn}
Let $T$ be a tile set that layer-computes the Boolean function $f : \{0,1\}^n\rightarrow\{0,1\}^n$ according to Definition~\ref{def:assemble a layer function}. 
Then for any $k\in\Nset$, $T$ also computes 
$f^k$.
%the $k$th iteration of~$f$ 
%$$ \underbrace{f(f(\ldots f(x))}_{k \text{ times}} = y \in \{0, 1\}^n$$ 
%in the sense that the terminal assembly of $\calT_x$ encodes $y$ along the glue curve $c + k \cdot \vec v$.
\end{lemma}
\begin{proof} 
We give a proof by induction on iteration $f^i$ for $i \in \{0,1,\ldots,k-2 \} $. 

For the base case, $i=0$, by Definition~\ref{def:assemble a layer function}, the seed $\sigma_x$ encodes $x\in\{ 0,1\}^n$ along $c$ using $\mathcal{G}_c(x)$ and places no tiles in $\mathrm{RHS}(c) \subsetneq \Rset^2$, hence $T$ computes $f^0(x)=x$.

Let $\vec{\alpha} = \alpha_0,\alpha_1,\ldots,\alpha_m$ be an assembly sequence of $\calT_x$ such that, inductively, we assume that in its final asembly $\alpha_m$ the cut $c + i \cdot \vec v$ encodes the bit sequence 
%$y' = \underbrace{f(f(\ldots f(x))}_{i \text{ times}} \in \{0, 1\}^n$, 
$y' = f^i(x) \in \{0, 1\}^n$ via $\mathcal{G}_c(f^i(x))$, 
and $\alpha_m$ has no tiles in $\mathrm{RHS}(c + i \cdot \vec v)$, and 
no tiles can stick in $\mathrm{LHS}(c + i \cdot \vec v)$.
Then, consider the seed assembly $\sigma_{y'}$ that encodes $y'$, and let 
$\vec{\alpha}_{y'}$ 
be the longest prefix of an assembly sequence that satisfies   
Definition~\ref{def:assemble a layer function}(\ref{def:condition:niceseq}) 
such that it does not place any tile in $\vec{\alpha}_{y'} |_{\mathrm{RHS}(c + \vec v)}$.
Running along each element of 
$\vec{\alpha}_{y'}$ in order, 
consider each tile $(t,z)$ that sticks (is attached) to the previous element of 
$\vec{\alpha}_{y'}$, and then consider the translated tile 
$(t,z + i\cdot \vec v)$.
Sticking these tiles in order, starting from $\vec\alpha_m$, yields\dwm{I am handwaving a little here. If I make it more formal, that may not halp the reader enough to be worth it.} an assembly sequence that ends with an assembly that encodes $f(y') = f^{i+1}(x)$ along the curve $c + (i+1)\cdot \vec v$ via $\mathcal{G}_{c + (i+1)\cdot \vec v}(f^{i+1}(x))$. 
This completes the induction.
\end{proof}


\newpage
\subsection{Self-assembled counters: impossibility results}

\begin{lemma}\label{lem:tiles to local circuit}
Let $T$ be a tile set that layer-computes the Boolean function $f : \{0,1\}^n\rightarrow\{0,1\}^n$ for $n \geq 4$.
Then there is a local circuit that computes $f$.
\end{lemma}
\begin{proof} 
First, some intuition:  the goal of the proof is to build an (exponentially large) circuit for $f$ by building one subcircuit for each input  $x\in \{0,1\}^n$, then appropriately wiring them together to get a circuit that computes $f$, and finally argue that the resulting circuit is local. We proceed as follows. 

For each input $x\in \{0,1\}^n$ let $\sigma_x$ be the seed assembly encoding $x$, and let $\calT_x=(T,\sigma_x,\tau)$, $c$, $\vec{v}$ be as defined in Definition~\ref{def:assemble a layer function}. 
We define a subcircuit $\calC_x$ as follows: 
Consider any assembly sequence $\vec{\alpha}$ of $\calT_x$ that satisfies Definition~\ref{def:assemble a layer function}(\ref{def:condition:niceseq}) and places no tiles in $\alpha |_{\mathrm{RHS}(c + \vec v)}$.
By directedness, all assembly sequences compute the same output for the layer, so the choice of $\vec{\alpha}$ over other assembly sequences is inconsequential.  % , and by Definition~\ref{def:bit encoding}, 
% We build a subcircuit as follows. 
For each tile attachment $t$ in $\vec{\alpha}$, add a gate, the gate inputs (wires) are the coordinates in $\Hset$ of the input glues to $t$, and the gate output wires are the coordinates of the other non-input glues of $t$. 
\dw{OK, I need to figure out how to interpret glues ``in the middle''... }
For every pair of co-located glues $g,g'$ in the assembly such that $\CS(g) = \CS(g')$ we add a wire from the gate output corresponding to $g$ to the gate input corresponding to $g'$.\footnote{Some gate inputs/outputs may not be joined up due to mismatches or unbound glues.}
\dw{Structural glues are ignored -- is it dangerous to go this road?} 
Each gate output is assigned a Boolean function (AND, OR, XOR, NOT, constant-0, constant-1, etc.) consistent with the bits assigned to wires/glues. 
Each gate that has at $\geq 1$ fanout has fanin $\leq 3$, and since $n\geq 4$, the circuit $\calC_x$ is local. 

Design another subcircuit $\calC_{=}$ that takes $n$ input bits and selects, for any input $x$, which circuit $\calC_x$ to activate.
$\calC_{=}$  can be implemented as a circuit of size $O(2^n  n)$ that has a lookup table encoded via constant 0/1 gates of all $2^n$ inputs of length $n$, and tests equality using a $2^n$ trees of depth $O(\log n)$ each.

The circuit $\calC$ is then defined to be $\calC_{=}$ appropriately wired to the $2^n$ subcircuits $\calC_x$ (one for each input $x$). 
\end{proof}


%
%\dw{Currently working on the following definition. the interesting thing is that I may not be forced to define a precise mapping to a local circuit, we simply need to show that for every   }
%\begin{definition}[Self-assembling a Boolean gate]
%Consider the set of assembly sequences that fill out a layer. 
%\end{definition}
%

 \begin{comment}
For $n\in\mathbb{N}, n \geq 2$ we define an assembly layer to be a width-1 

We define a {\em base-$b$ layered counter} to be an $n \times \lceil log_b n \rceil $ assembly made of successive arbitrary-height-n and 1-tile-wide layers of tiles. Each glue is labeled with a symbol (in the "binary counter" case the symbols are {0,1}). The "output of the counter" is the glue sequence of "glue columns" along the border of each layer, similar to a circuit but with glues instead of wires.

We convert any counter to a layered circuit: 

Two cases (actually there will be only one case, but it is illustrative for our discussion here to first show an easy case):

1. Suppose the growth frontier is always of size 1 (an easy, quite illustrative, case)
 - Examine any assembly sequence, starting at step t=0 (first tile attachment to seed).
 - for any t \leq circuit_size, look at the tile attachment event A_t, and create a new gate G_t. 
 - The inputs to G_t correspond to input glues*** of A_t, and outputs of G_t are the non-input glues of A_t (wires use the same naming convention as glues, etc.).
Since the growth frontier is of size 1, 

2. Suppose not, i.e. the growth frontier is not always of size 1. In all growth sequences, if there is a well-defined set of inputs sides and output sides for each tile, just use the above approach. 

Since the counter is directed, there is a single final assembly and we can look at the glues there. 



** A counter 
*** Input glues are well-defined for each tile in the (unique) assembly sequence. (Note that this is not the case  


\end{comment}



\begin{theorem}\label{thm:self-assembly:no max counter}
Let $n\in \{4,5,\ldots \}$.
There is no tile set $T$ that self-assembles a $2^n$ counter on $n$-bits: meaning that it assembles $2^n$ iterations of a bijective, or a quasi bijective, layer-function $f : \{0,1\}^n \rightarrow \{0,1\}^n$. 
\end{theorem}
\begin{proof}
By Lemma~\ref{lem:tiles to local circuit} there is a local circuit $\calC$ that layer-computes the same function, $f$, as  $T$.
By Theorem~\ref{th:main}, $\calC$ does not   
compute $2^n$ iterations of neither a  bijective, nor a quasi bijective, layer-function $f$ on $n$ bits.
\end{proof}






%\color{blue}
%Rough work from here on.
%
%
%How do organise things?
%
%Seems I need to define a wide class of self-assembled $k$-counters. 
%
%Then show that any tile set that implements  a $k$-counter is in fact implementing a local iterated function / local circuit. Since such a counter would violate the even bijection property of local circuits it can not be implemented.  
%
%\begin{lemma}
%There is no tile set $T$ such that 
%\end{lemma}
%
%A ``happy''\dwm{temporary name, for fun}  maximal-$n$-bit-counter is an aTAM system $\calT$ that is directed, ... meets the conditions of being mappable to a circuit.... counts to $2^n$.
%
%\begin{itemize}
%\item ``Happy'' counters can not compute odd bijections
%\item ``Happy'' quasi-counters can not compute odd bijections
%\end{itemize}
%

\color{blue}
\subsection{Self-assembled counters: discussion and future work}

Some points to cover: 

The result holds no matter how deep the layer. E.g. for the multilayer def of IBCs in \cite{WoodsDotyWinfree} (SI, Section ??). 

In particular, this implies that 2-bit zig-zag counters~\cite{}, or 2-bit IBC counters~\cite{WoodsDotyWinfree} are impossible.  

The requirement of locality in circuits seems reasonable in the context of self-assembly. 


%  is less clear is how to consider (or what we can prove about) other reasonable kinds of systems, in particular those that have different growth patterns (e.g. different orders of tiling the a rectangle) on different inputs. 

Future work would be to show if there are any features of self-assembly can be applied to compute odd bijections (such as $b^n$ counters for some $b\geq 2$.
\begin{itemize}
\item larger alphabet, in particular odd-size alphabet~\cite{jarrko}
\item Undirected counter systems
\item What about systems that use the same tile set in each ``layer'' but different orders of growth depending on the input to the layer? 
% arbitrary growth-order systems, in particular where there the mapping from the set of all terminal assemblies to a single, repeated-layer, Boolean circuit is not the direct mapping we used here.
\end{itemize}


\dw{2020-4-18: The below point was made a few years ago but we now know a little more. Multi-layer circuits can cheat by having extra ``ignored configurations'', so our techniques may not prevent them from making counters. In the 6-bit IBC case 1 layer and 2 layer can not do a counter, but for 3-layer our negative result does not apply.  It might be worth showing a positive result on that?}
Multi-layer \ibcs, as well as alphabet size $>2$ \ibcs, are straightforward to define~\cite{WoodsDotyWinfree}. Although they've not been experimentally implemented it is within the realm of possibility to do so; requiring more (DNA) tile types than the single-layer/size-$2$ alphabet case. It would be interesting to see whether or not our techniques could be generalised to either or both of the cases of multi-layer or/and randomised circuits. It seems likely that these generalisations of the model would confer more power, but characterising their power remains open. Indeed if that were the case, the present paper shows the necessity of generalising the model somehow in order to circumvent the limitations we show here. For example, do 2-layer \ibcs with alphabet $\{0,1\}$ exhibit a $2^n$-counter?
Do single-layer \ibcs with alphabet size $|\Sigma|>2$ exhibit a $|\Sigma|^n$-counter?\ (It is not difficult to show  that alphabet size $3$ permits $2^n$ counters.) \dwm{todo: check this!}


\color{black}

